Learning Personalized Representations using Graph Convolutional Network

Generating representations that precisely reflect customers' behavior is an important task for providing personalized skill routing experience in Alexa. Currently, Dynamic Routing (DR) team, which is responsible for routing Alexa traffic to providers or skills, relies on two features to be served as personal signals: absolute traffic count and normalized traffic count of every skill usage per customer. Neither of them considers the network based structure for interactions between customers and skills, which contain richer information for customer preferences. In this work, we first build a heterogeneous edge attributed graph based customers' past interactions with the invoked skills, in which the user requests (utterances) are modeled as edges. Then we propose a graph convolutional network(GCN) based model, namely Personalized Dynamic Routing Feature Encoder(PDRFE), that generates personalized customer representations learned from the built graph. Compared with existing models, PDRFE is able to further capture contextual information in the graph convolutional function. The performance of our proposed model is evaluated by a downstream task, defect prediction, that predicts the defect label from the learned embeddings of customers and their triggered skills. We observe up to 41% improvements on the cross entropy metric for our proposed models compared to the baselines.

==> backup.tex <==
\section{NEED ORGANIZATION}

[Image: image.png]
One direction to consider is making such improvements within the scope of representation learning/ neural embedding, which will be subsequently incorporated into HypRank. The reasons we do not prefer to touch the structure of HypRank model are two fold: 1. From the engineering side, HypRank model has been extensively tested and verified at service level. It is not guaranteed that a new model will compete with its speed and stability. 2. From the data analysis side, as pointed out in https://quip-amazon.com/c09UARe2GUIb that customer historic behavior contains rich information of personal preferences and behavioral patterns that are correlated with the invoked skills. However, the current HypRank model does not consider well this aspect for its model inputs. As a result, considering algorithms to improve the Hyprank model by providing a set of input embeddings will avoid the risk of service level performance for Alexa and at the same time introduce customers’ behavior patterns to HypRank. 

In the following, we will define our problem in the scope of representation learning.

Problem Formulation

Since Graph Convolutional Network (GCN) is a popular tool in modeling the interaction-based relationships (e.g. user-skill interaction graph in our case), we decide to formulate this representation learning problem within the GCN framework to make it concise.

Given a user-skill interaction bipartite graph G=(V,E) where V is the set of vertices and E is the set of edges linking the nodes. Here V={U,S} where U refers to the set of user nodes and S refers to the set of skill nodes. And e∈E exists between a user u∈U and a skill s∈S only when the the request of u is fulfilled by the skill s, which is also denoted by eu,s​. The objective is to design a model f that maps the input node feature (hu0​,eu,s​,hs0​) of graph to a set of embedding vectors for both the user and skill nodes, denoted as huL​=f(hu0​,eu,s​,hs0​) and hsL​=f(hs0​,es,u​,hu0​), respectively, such that when incorporating these embeddings to some downstream tasks, their corresponding performances are maximized. 

Input: G
Output:  huL​,hsL​

Downstream Task 1 is defect prediction with the following objective,

minσ​∣E∣1​∑u∈U,s∈S​CE(σ(huL​,hsL​),yCPDR​),

where σ(⋅,⋅)is the edge classification predictor function. This can be any classifier that takes the embeddings for both skill and user nodes. Here yCPDR​ is the defect label from CPDR, and CE(⋅)is the cross-entropy.




Reasons/Connections : Since the embeddings eventually serve for HypRank, it is intuitive to choose downstream task that is closely related the objectives in HypRank. In this way, a set of embeddings that perform well in this defect prediction task could possibly provide improvements when incorporating them into HypRank because we believe the richness of the information encoded into the embedding vector can be reflected by this defect prediction task.


Downstream Task 2 is the contrastive loss.

∑s∈S1p​;s~,s^∈S3p​​−logexp(sim(hsL​,hs^L​)/τ)exp(sim(hsL​,hs~L​)/τ)​

Where “sim” refers to similarity measure between the input embeddings. τis a constant hyperparameter. s,s~ are similar skills in 1p and 3p. s,s^ are different skills in 1p and 3p.

Reasons/Connections: We want to measure the closeness between the similar 1p and 3p skill embeddings. If the above loss is small, it means the similar 1p and 3p skills are close in the embedding space, and different 1p and 3p skills are far away in the embedding space. As a result, when incorporating such embeddings into HypRank model, there should be less bias towards 1p skill, which subsequently increase 3p traffic.

Ideally, if two skills are providing the similar functionality, two skills should be located closely to each other in the embedding space. On the contrary, if two skills are providing the different functionality, two skills should be located a bit far away to each other in the embedding space. However, this relationship is not quickly captured in the GCN, especially in our application.

The idea behind of GCN is passing the information through the edge, which is interaction history in our case. Thus, the embedding of a skill is slowly propagated (or making impact) to user node and then information is propagated to other skill node. This means that the propagation (speed) of information among skills highly depends on the co-invocated relationship. If there is vast amount of user who invoked both of two skills, the information propagation between two skills are accelerated than the average. If not, it takes time to reflect the relationship between skill. Unfortunately, the latter is the case in our application. If two skills are providing the similar function, people tends to use only one of them rather both of them. Thus, connectivity between these two skill is really scarce in terms of co-invoke customer. For example, “Big sky” and “Weather” provide almost similar functionality, but there are only few amount of user who use both of the skills.

For this reason, if we can directly consider the skill-skill relationship, it will help to get the more accurate embedding within the limited amount of time.

Downstream Task 3 is the margin loss in the link prediction:

∑u∈U,s∈S,s~∈Neg(U)​max(M−<huL​,hsL​>+<huL​,hs~L​>,0),

where Neg(U) is the randomly sampled noise skill sets with nodes connected to u∈U. M is a constant hyperparameter. This is also a revised PinSage loss since the original version in PinSage considers only nodes of same types. 

Reasons/Connections:A good embedding should naturally reflect the connectivity between nodes in the graph. If this loss is small with the proposed embedding inputs, then it validates that the embeddings should be able to used for link prediction (recommendation), a natural task that is similar to the one for HypRank. Hence, it should possibly work for HypRank model as well. 


Benchmark



1. Model side

As previously mentioned, we are tackling this problem within the GCN framework. There are several models that we found can be used as our baseline models. We choose the models based on the following factors: 1. If the model is one of the SOTA models that works with heterogeneous graph; 2. If the model is one of the SOTA models designed for large scale scenarios; 3. If the SOTA model that considers edge attributes. The reason we choose these three criterias is because we want to make sure that the scenarios to which baseline models are applied can mimic the real-life scenarios that Alexa is facing (e.g. large scale user-Alexa interactions, heterogeneous graph properties, consider metadata from utterance to be some edge attributes). Here we select several baselines and each of them corresponds to one or multiple factors listed above.  However, it is noteworthy that none of the baselines we found below are 100 % designed for our problems from the objective side. As a result, in order to make them become baselines in our scenario, proper changes to e.g. loss objectives are necessary.


1. PinSage (https://github.com/dmlc/dgl/tree/master/examples/pytorch/pinsage) (large scale, random walk sampler)
    1. Coded to be able to handle hetero graph (for both user & skill nodes)
    2. working on sampler part
2. Heterogeneous Graph Transformer (https://github.com/dmlc/dgl/tree/master/examples/pytorch/hgt) ( heterogeneous, large scale)
    1. Coded to fit our data (currently doesn’t involve edge attribute message passing)
3. Heterogeneous Graph Attention Network (https://github.com/dmlc/dgl/tree/master/examples/pytorch/han)( heterogeneous, large scale)
4. A Generalization of Transformer Networks (https://github.com/graphdeeplearning/graphtransformer) (heterogeneous, large scale, edge attributes)


To remember that GCN is not the only option for this task, there are others such as matrix-factorization based and neural network based models with which the same objectives (previously mentioned) can be considered. As a result, we also want to include a few of these models to our baseline to compare the performance between the GCN-based models and models of other types.

https://arxiv.org/pdf/2002.11522.pdf



1. Online Learning for Latent Dirichlet Allocation (https://github.com/dmlc/dgl/tree/master/examples/pytorch/lda)
2. Multi Layer Perceptron (MLP)
3. matrix factorization










DO NOT READ

The end (ignore texts below)








such that when incorporating the embeddings into HypRank, the defect rate is minimized. Here we use this simplified notation to representation the HypRank model taking the embedding vectors hu​ and hs​ as input and outputting the defect indicator HR:Rn×Rn↦{0,1} . Then the problem objective is defined as follow:


minf​∣U∣1​∑∀u∈U​∑∀s∈N(u)​1∑∀s∈N(u)​HR(huL​,hsL​)​



However, directly minimizing this objective is infeasible since when f is updated, the HR needs to be updated as well to fit for the new embeddings from f. To avoid this issue and to focus more on the, we introduce alternative objectives to directly focus on minimizing f while ignoring the HR










1. 










and the traffic for a 3p skill, TA(s), is maximized for ∀s∈S3p​. Here S3p​⊂Sis a subset of S that contains only 3p skills.  Here N(u)is a set including all skill nodes that are invoked by u. And

DR(u)=∑∀s∈N(u)​1∑∀s∈N(u)​Indicator{defect(s)=1}​ ,
TA(s)=∑∀s~∼s,s~∈S​1∑∀s~∼s,s~∈S1p​​1​.



[Image: image.png]
 


1. 


Implementation details 


1. Parallel Edge Attributes 
2. Incorporate node/edge features with different baseline models
3. Prepare train/val/test sets



TODO:

1. problem - embeddings
2. why to choose those losses






Model Design

Option 1: Contrastive loss.

In representation learning with bipartite graph, 


∑s∈S1p​;s~,s^∈S3p​​−logexp(sim(hsL​,hs^L​)/τ)exp(sim(hsL​,hs~L​)/τ)​

Where “sim” refers to similarity measure between the input embeddings. τis a constant hyperparameter. s,s~ are similar skills in 1p and 3p. s,s^ are different skills in 1p and 3p.

Reasons/Connections: We want to measure the closeness between the similar 1p and 3p skill embeddings. If the above loss is small, it means the similar 1p and 3p skills are close in the embedding space, and different 1p and 3p skills are far away in the embedding space. As a result, when incorporating such embeddings into HypRank model, there should be less bias towards 1p skill, which subsequently increase 3p traffic.

Ideally, if two skills are providing the similar functionality, two skills should be located closely to each other in the embedding space. On the contrary, if two skills are providing the different functionality, two skills should be located a bit far away to each other in the embedding space. However, this relationship is not quickly captured in the GCN, especially in our application.

The idea behind of GCN is passing the information through the edge, which is interaction history in our case. Thus, the embedding of a skill is slowly propagated (or making impact) to user node and then information is propagated to other skill node. This means that the propagation (speed) of information among skills highly depends on the co-invocated relationship. If there is vast amount of user who invoked both of two skills, the information propagation between two skills are accelerated than the average. If not, it takes time to reflect the relationship between skill. Unfortunately, the latter is the case in our application. If two skills are providing the similar function, people tends to use only one of them rather both of them. Thus, connectivity between these two skill is really scarce in terms of co-invoke customer. For example, “Big sky” and “Weather” provide almost similar functionality, but there are only few amount of user who use both of the skills.

For this reason, if we can directly consider the skill-skill relationship, it will help to get the more accurate embedding within the limited amount of time.

Option2: The link prediction loss:

∑u∈U,s∈S,s~∈Neg(U)​max(M−<huL​,hsL​>+<huL​,hs~L​>,0),

where Neg(U) is the randomly sampled noise skill sets with nodes connected to u∈U. M is a constant hyperparameter. This is also a revised PinSage loss since the original version in PinSage considers only nodes of same types. 

Reasons/Connections: A good embedding should naturally reflect the connectivity between nodes in the graph. Which means the connnected nodes should have closed embeddings than unconnected nodes. 






\section{problem statement}

Problem Statement

Since Graph Convolutional Network (GCN) is a popular tool in modeling the interaction-based relationships (e.g. user-skill interaction graph in our case), we decide to formulate this problem as a representation learning problem and formulate it within the GCN framework to make it concise.

Given a user-skill interaction bipartite graph G=(V,E) where V is the set of vertices and E is the set of edges linking the nodes. Here V={U,S} where U refers to the set of user nodes and S refers to the set of skill nodes. And eu,s​∈E exists between a user u∈U and a skill s∈S only when the the request of u is fulfilled by the skill s. And eu,s​=(yu,sCPDR​,uttu,s​) is the tuple recording the defect label yu,sCPDR​ (either soft or hard-coded labels from CPDR) and the utterance uttu,s​ between user u and skill s. The objective is to design a model f that maps the input node feature (hu0​,eu,s​,hs0​) of graph to a set of embedding vectors for both the user and skill nodes, denoted as huL​=f(hu0​,eu,s​,hs0​) and hsL​=f(hs0​,es,u​,hu0​), respectively, such that when incorporating these embeddings to some downstream tasks, their corresponding performances are maximized. 

Input: G
Output:  huL​,hsL​

Downstream Task: Defect prediction with the following objective,

minσ​∣E∣1​∑eu,s​∈E​CE(σ(huL​,hsL​),yu,sCPDR​),

where $\sigma(⋅,⋅)$ is the edge classification predictor function. This can be any classifier that takes the embeddings for both skill and user nodes. CE(⋅)is the cross-entropy.

Reasons/Connections : Since the embeddings eventually serve for HypRank, it is intuitive to choose downstream task that is closely related the objectives in HypRank. In this way, a set of embeddings that perform well in this defect prediction task could possibly provide improvements when incorporating them into HypRank because we believe the richness of the information encoded into the embedding vector for HypRank can be reflected by this defect prediction task.

\section{losses}

Loss Objective

Introduction

Here we introduce different loss objectives as described in https://quip-amazon.com/KCEKAu3Z4cQX. To make consistent notations we repeat the description of variables as described in https://quip-amazon.com/5l26ATgp1jA8


Given a user-skill interaction bipartite graph G=(V,E) where V is the set of vertices and E is the set of edges linking the nodes. Here V={U,S} where U refers to the set of user nodes and S refers to the set of skill nodes. And eu,s​∈E exists between a user u∈U and a skill s∈S only when the the request of u is fulfilled by the skill s. And eu,s​=(yu,sCPDR​,uttu,s​) is the tuple recording the defect label yu,sCPDR​ (either soft or hard-coded labels from CPDR) and the utterance uttu,s​ between user u and skill s. The objective is to design a model f that maps the input node feature (hu0​,eu,s​,hs0​) of graph to a set of embedding vectors for both the user and skill nodes, denoted as huL​=f(hu0​,eu,s​,hs0​) and hsL​=f(hs0​,es,u​,hu0​), respectively, such that when incorporating these embeddings to some downstream tasks, their corresponding performances are maximized. 

Input: G
Output:  huL​,hsL​


Loss Objectives

The loss objectives are described below with each loss function followed by a description of its rationales.

Objective 1.1:  skill-skill node similarity/dissimilarity loss

∑u∈U​∑s1​,s2​∈N(u),s~∈S∖N(u)​max(M−<hs1​L​,hs2​L​>+<hs1​L​,hs~L​>,0),

where N(u) is the set of skill nodes that are connected with the user node u. M is a constant hyperparameter. This is also the original PinSage loss.

Reasons/Connections: A good embedding should naturally reflect the connectivity between nodes in the graph. Here if two skill nodes that are connected with the same user node, then we should naturally make their embeddings closer. In contrast, if the two skill nodes are not connected via a user node, we should make their embeddings far away. 

Objective 1.2:  user-user node similarity/dissimilarity loss

∑s∈S​∑u1​,u2​∈N(s),u~∈U∖N(s)​max(M−<hu1​L​,hu2​L​>+<hu1​L​,hu~L​>,0),

This is similar to the previous loss but works with user node

Reasons/Connections: The same intuition as before but works with user nodes 


Objective  1.3: user-skill node similarity/dissimilarity loss

∑u∈U​∑s∈S,s~∈Neg(u)​max(M−<huL​,hsL​>+<huL​,hs~L​>,0),

where Neg(u) is the set of randomly sampled noise skill nodes that are not connected to the user node u. M is a constant hyperparameter. 

Reasons/Connections: Similar intuition as before. If a user invokes a particular loss, their embeddings should be closer than the embeddings between the unconnected user and skill nodes. 


Objective  1.4: Defect based user-skill node similarity/dissimilarity loss:

∑eu,s​∈E∖Edefect​,eu,s~​∈Edefect​​max(M−<huL​,hsL​>+<huL​,hs~L​>,0),

where Edefect​ is the set of edges with edge attribute yCPDR=1. 

Reasons/Connections: Here we want to make sure the embeddings of connected nodes between non-defected edges to be closer than that for defected edges.


Objective 2 https://quip-amazon.com/5l26ATgp1jA8#BGB9CAGNVtQ: 

∑s∈S1p​;s~,s^∈S3p​​−logexp(sim(hsL​,hs^L​)/τ)exp(sim(hsL​,hs~L​)/τ)​

Where “sim” refers to similarity measure between the input embeddings. τis a constant hyperparameter. s,s~ are similar skills in 1p and 3p. s,s^ are different skills in 1p and 3p, respectively. Here we measure the similarity between different skill nodes by the following function:

f(s1​,s2​)=sign(maxa∈UTTs1​p​,b∈UTTs3​p​​cosinesimilarity(a,b)+ρ), 

where UTTs​ refers to the set of embeddings for the utterance that is connected to node s. If the above function equals to 1, which means the two skill nodes are semantically similar. Otherwise if the function equals to -1, the two skill nodes are different. ρ is a constant parameter for adjustment. If a node 

Reasons/Connections: We want to measure the closeness between the similar 1p and 3p skill embeddings. If the above loss is small, it means the similar 1p and 3p skills are close in the embedding space, and different 1p and 3p skills are far away in the embedding space. As a result, when incorporating such embeddings into HypRank model, there should be less bias towards 1p skill, which subsequently increase 3p traffic.

Remark. Note that it’s not necessary that the distance measure has to be cosine similarity. One can use arbitrary distance measure. 







P.S. Some explorations for similarity measure part with utterance embedding: https://quip-amazon.com/jI4iA6Qd62HC. This is to check which type of embedding models can generate utterance embeddings to reflect the semantic closeness between skills. 

Conclusion: Public pre-trained model for sentence did not perform very well with our dataset. This is possibly due to that our utterance are with similar lengths and are short. Which will result in closed embeddings between two sentences regardless of their semantic information. We can try to use HypRank sub-module to generate embeddings or we can fine-tune the public model with our utterance dataset in a self-supervised way.



==> conclusion.tex <==
In this work, we build a heterogeneous graph with attributed edges based on customers' past interactions with the invoked skills. Besides, we propose PDRFE, a GCN-based representation learning model, designed for generating personalized customer-skill embeddings from the built graph. The proposed model is evalulated according to a binary classification downstream task, known as defect prediction, which reflects the customer's preferences to the skills. We compare our models to the proposed baselines and observed up to 41\% improvement in the cross-entropy in the downstream evaluation. Additionally, an ablation study is included to understand the performance contribution of the modules in PDRFE where the resulting improvements range from 12\% to 19\%. 


%TT, I agree with sz, this paragraph is not needed. I re-wrote the next one and added it to the paragraph below. 
%It is noteworthy that one of the Amazon 14 leadership principles is customer obsession, which instructs Amazonians to work vigorously to earn and keep customer trust. \sz{remove this sentence} \hs{why we remove this? I feel the connection would miss if this one is removed.} \sz{I think everyone in Amazon should know it, no need to notice.} \hs{But I feel making this statement here could make the transition between paragraphs smoother}
%In our case, this can be interpreted as how to provide improvements to improve customer satisfactions? Or more specifically, how to reduce the defect rate during the fulfillment of a user’s request with Alexa's skills. 


Our PDRFE model impacts customer experience and improves downstream customer satisfaction by reducing the defect rate during fulfillment of a user's request by Alexa's skills. We demonstrate that PDRFE model generates more precise customer and skill representations which encodes customer-skill relationship, resulting in lower cross-entropy in the defect prediction. As a result, such characterization of customer-skill connectivity by PDRFE can be possibly applied to the existing Alexa DR tools in order to improve the accuracy of the current routing services. For example, it can benefit Alexa DR's ranking model (HypRank~\cite{kim2018scalable}) which considers joining the information from the user side such as utterance, interpretation, etc and forms hypothesis to re-rank the existing skill candidates to find the most likely skill to answer user’s request. It reduces the defect rate while answering users’ requests. However, this model does not consider the customer and skill interactions as a graph, which means the current representations in HypRank may not reflect the natural interactions between customers and skills. In the future work, we plan to inject the representations from the proposed PDRFE model to provide more contextual information for the customers and skills to reflect their natural connectivity into HypRank ranking decisions.

%\sz{changed verbs to present tense, in order be consistent with others. Make clear what is future work}

==> introduction.tex <==
The advancement of Alexa AI technologies enable customers to have various options for interacting with Alexa devices. For example, a person can ask Echo to play a song, to turn on a TV, or to open air conditioners while being away from home. Alexa provides such convenience to help people automate daily tasks with ease. So far, Alexa AI has created more than 200k different skills that range from video display, automatic subscriptions to home services and etc. Such services cover almost every possible task in customer's daily life. Providing such high-end services with Alexa has also attracted nearly 800 million registered users generating about 500 million user-Alexa interactions daily.

One of the core concepts behind Alexa services is the representation learning models created by Alexa Dynamic Routing (Alexa DR) team. Alexa DR develops ranking models and rules to generate representations  of the skills and use these representations to rank each skill for every customer's request. Subsequently, customers' requests can be routed to the skills that can response to those requests.
Recently, Alexa DR starts to extend its ranking models to consider customer-skill interactions by using simple features such as normalized impression counts of successful customer interactions with skills as input features to its ranking models. However, these simple features are not strong enough to fully encode the complex nature of customer-skill interactions. For example, a simple impression count hardly captures the similarity between the skills, and thus looses its predictive power in that regard.
Another pitfall is that simple features are computed and used without any consideration on the context. For example, the normalized traffic count for a pair of customer and skill is invariant to the utterance text. 

%\sz{We should describe the advantage of graph structure, before describing models. Filled the gap and refactored the following paragraph.} 
In this work, taking into account the above considerations, we propose to model such interactions in a bipartite graph structure with heterogeneous node types (user nodes and skill nodes). Besides, we further consider adding the utterances as edge features in order to capture the contextual information between customers and skills in the graph.
Inspired by recent advance in graph modeling, we propose to utilize GCN models in our problem. Previous studies have widely demonstrated the superior performance of graph modeling on encoding interactions between two or more entities~\cite{DBLP:journals/debu/HamiltonYL17,schlichtkrull2018modeling,wang2018deep,velivckovic2017graph,wang2019kgat,wang2019heterogeneous}, and hence provides a natural mechanism to consider context information during modeling through edge-based convolution operations~\cite{li2019spam,gong2019exploiting,hu2020heterogeneous,dwivedi2020generalization}.

However, there is one limitation in the existing GCN models for our particular setup. Namely, the conventional GCN models lack consideration on edge attribute in characterizing the relation between the customer and the skill nodes.
For example, in link prediction formulation (Section~\ref{problem_define}), the edge between customer and skill is predicted only by the customer and skill embedding.
Thus, a customer will have the same edge probability to a certain skill regardless of the utterance text, which does not make sense in our application. Given different customers and the same utterance, the probability of matching the customers to a certain skill should be different. This should also hold in the case where the probabilities for the match of skills to a certain customer given different utterances. To remedy this problem, either the customer or skill embedding needs to be further adjusted to reflect the utterance text.

%  propagate all of the connecting edge information to enrich the node embeddings.
% For instance, to update the embedding of a customer, all of his/her requests (e.g. utterances) are considered simultaneously during message passing stage in GCN.
% Although the embeddings of the customer is enriched in this way, such propagation of edge information does not reflect the customer's preference to skills. Take our Alexa service as an example,
% A customer can invoke the skill ``Weather" by saying ``What's the weather like?", or invoke another skill ``Communication" by ``Drop in all devices.". Without considering individual edge information (e.g. utterances), such difference between customers and skills cannot be distinguished.
%  This is because the utterances are used only for updating the embedding of the customer node, and there is no characterization on the preferences between the customer and the related skills.

% For instance, to update the embedding of a customer, all of his/her requests (e.g. utterances) are considered.
% Although the embeddings of the customer is enriched, such consideration of edge information does not reflect the customer's preference to skills.
% This is because the utterances are used only for updating the embedding of the customer node, and there is no characterization on the preferences between the customer and the related skills.
% \jo{@Hongyu: this must be about the attention right? And the attention is applied per traffic right?}
%\jo{Tara Taghavi: @Hongyu: I can read only one limitations above, the fact that customer preference for a skill is not considered, what is the other limitation?}

To overcome this issue, we propose a model, named Personalized Dynamic Routing Feature Encoder (PDRFE), that aims to generate personalized embeddings for the customer nodes given the customer and his/her triggering utterances for different skills. PDRFE includes a mechanism, which is denoted as \textit{personalizer}, to provide customer embeddings adjusted with respect to the utterance text. Besides, we also consider two other modules in PDRFE to further improve the model performance by considering the edge features. The first one is the edge-based attention module. PDRFE applies attention module to distinguish the important connection and update the customer embedding and skill embedding accordingly. This is because some skills are designed to be more interactive than others, and create more frequent but less important request such as "next", "repeat the question". Thus, importance of edge needs to be distinguished and weighted differently to precisely capture the customer's true preference to skills. The second module is the edge convolution that considers all the edge features in updating the corresponding node embedding. In our case in Alexa, the edge features (e.g. utterances) indicate the customers behaviours to their invoked skills. And it also helps identifying the difference between skills. As a result, it is natural to consider the edge information in updating the node embedddings for both the customers and skills. Overall, we compare our proposed model with 4 baselines with a downstream evaluation task (defect prediction) that predicts the defect label from the personalized embedding of customers and the embedding of their triggering skills.
Additionally, we also provide ablation study for the modules we proposed in PDRFE to help identify the contribution of sub-modules to the downstream task.



% First, existing state-of-the-art edge-based operators such as~\cite{hu2020heterogeneous,dwivedi2020generalization} weight all of the connecting edge information to be the same. 
% This is not true in Alexa service.



% However, there is a limitation in the existing GCN models for our particular setup.
% First, existing state-of-the-art edge-based operators such as~\cite{hu2020heterogeneous,dwivedi2020generalization} weight all of the connecting edge information to be the same. 
% This is not true in Alexa service.
% Some skills are designed to be more interactive than others, and create more frequent but less important request such as "next", "repeat the question".
% Thus, importance of edge needs to be distinguished and weighted differently to precisely capture the customer's true preference to skills.may have the same edge probability to a certain skill regardless of the utterance text, which does not make sense in our application.
% To remedy this problem, either the customer or skill embedding needs to be further adjusted to reflect the utterance text

% %  propagate all of the connecting edge information to enrich the node embeddings.
% % For instance, to update the embedding of a customer, all of his/her requests (e.g. utterances) are considered simultaneously during message passing stage in GCN.
% % Although the embeddings of the customer is enriched in this way, such propagation of edge information does not reflect the customer's preference to skills. Take our Alexa service as an example,
% % A customer can invoke the skill ``Weather" by saying ``What's the weather like?", or invoke another skill ``Communication" by ``Drop in all devices.". Without considering individual edge information (e.g. utterances), such difference between customers and skills cannot be distinguished.
% %  This is because the utterances are used only for updating the embedding of the customer node, and there is no characterization on the preferences between the customer and the related skills.

% % For instance, to update the embedding of a customer, all of his/her requests (e.g. utterances) are considered.
% % Although the embeddings of the customer is enriched, such consideration of edge information does not reflect the customer's preference to skills.
% % This is because the utterances are used only for updating the embedding of the customer node, and there is no characterization on the preferences between the customer and the related skills.
% % \jo{@Hongyu: this must be about the attention right? And the attention is applied per traffic right?}
% %\jo{Tara Taghavi: @Hongyu: I can read only one limitations above, the fact that customer preference for a skill is not considered, what is the other limitation?}

% To overcome this issue, we propose a model, named Personalized Dynamic Routing Feature Encoder (PDRFE), that aims to generate personalized embeddings for the customer nodes given the customer and his/her triggering utterances for different skills. 
% PDRFE applies attention module to distinguish the important connection and update the customer embedding and skill embedding accordingly.
% In addition, PDRFE includes a mechanism, which is denoted as \textit{personalizer}, to provide customer embeddings adjusted with respect to the utterance text.
% We compare our proposed model with 4 baselines with a downstream evaluation task (defect prediction) that predicts the defect label from the personalized embedding of customers and the embedding of their triggering skills.
% Additionally, we also provide ablation study for the modules we proposed in PDRFE to help identify the contribution of sub-modules to the downstream task.

We organized the paper as follows: We first discuss problem setup and the proposed PDRFE model in the next section, followed by the experiment section that includes experiment setup, the comparison results between PDRFE and the 4 baseline models through a downstream task evaluation, as well as ablation studies for PDRFE. Finally, we conclude our study and explicitly state the customer impact of this study for Amazon.

==> method.tex <==
Here we describe the structures of the proposed PDRFE model. Specifically, it involves 3 major components: 1) An encoder for edge attributes 2) An Edge-based convolution operator in GCN that updates the embedding $(\textbf{h}_u, \textbf{h}_s)$ 3) A personalizer designed for generating personalized customer embedding that reflects the customer's requests.
% [PENDING] 4. Contrastive learning constraint for the skill ambiguity issue. 

\subsection{Encoder for Edge Attributes}
% \sout{In the common case [some citations], the edge features are encoded along the update of the node features.
% In our case, however, we choose to use the fixed edge features generated by a submodule in HypRank by taking the utterances as inputs.
% HypRank is a model~\cite{kim2018scalable} [some citation and explanation].
% The reason we choose to use fixed edge features rather than updating these features during training is because the edge features should correctly reflect the closeness between utterances.
% Similar utterances should be closer in the feature space than those of dissimilar utterances. Without carefully setup the constraints during the representation learning, it is hard to achieve this goal.
% However, on the other hand, the outputting features from HypRank are able to reflect such utterance similarity by its design.
% Hence, adopting the utterance embeddings from HypRank is a straightforward choice.
% Another subsequent benefit comes from the choice of HypRank is the training complexity, since the utterance embeddings are pre-computed before training.}
In this work, the primary edge attribute is the utterance text. We use a pre-trained Bi-LSTM text encoder to convert this utterance to feature vector, and there are three reasons.
First, our focus is about the interaction and not the semantic meaning of the utterance.
Thus, if it is carelessly trained from the scratch, there is a risk that the learned text encoder does not fully reflect semantic meaning of the utterance.
Second, using a pre-trained model reduces complexity in training and enables quicker iterations.
Third, using the Bi-LSTM over the other structures is to capture the cross-hypothesis correlation, which is an intermediate for generating utterance embeddings~\cite{kim2018scalable}.
Please note that this pre-trained model is the one shared within Alexa DR, hence the performance of this model has already been fully tested in production.

%Directly adopting the embeddings avoids the aforementioned pitfall and to reduce the training complexity, by fixing the utterance embedidng, we choose to use  caused by %To avoid introducing extra uncertainty caused by learning new edge features with extra constraints, we choose to encode edge features by the pre-trained HypRank model instead. %\sz{this sentence is confusing, please be more precise.}

\subsection{Edge-based Convolution Operator}
% In contrast to the personalizer, which is built on top of the last layer in GCN, Edge-based convolution operator is built during the message propagation stage.  \sz{what's the goal of edge-based conlution operator? is it the same with personalizer?}
Edge-based Convolution operators allow the propagation of the edge features to all of its connected neighboring nodes. It is known that considering edge features during graph convolution usually enriches the information for the nodes because such edge information characterizes the natural interaction between the connected nodes~\cite{gilmer2017neural,gong2019exploiting,dwivedi2020generalization}. For example, an edge can record the bond types in a molecular graph, the rating scores in a user-movie social media graph, or the contextual information in our customer-skill graph in Alexa, etc. To improve the performance of our model, we explore two edge-based convolution operators.
%\sz{Usually we propose two types of models when we can't decide which one is better except experiments. Is it that case here?}
%\hs{Still in progress}
%\sz{Did you take a sampling function in the neighbor nodes? Please describe.} /hs{there's no specific sampling function for edge-based convolution, so just ignored this comment} \sz{that's actually an advantage of our proposed model that we should describe in the paper.}


\textbf{\emph{NNConv:}} NNConv is proposed in the Message Passing Neural Network designed to infer quantum properties of molecules based on the structure of the molecules and their bond types (e.g. edge features)~\cite{gilmer2017neural}.
It demonstrates the superior performance to the corresponding baselines in terms of the inferences on quantum properties by considering the edge features in GCN message passing stage.
Analogous to their setup, where customer and skill nodes refer to the vertices of molecules and utterances refer to the the bond types, we choose to apply this module in the proposed PDRFE model.
For completeness, the message passing function is shown in Eq.~\ref{NNConv}:
\begin{equation}
\label{NNConv}
\textbf{h}_{i}^{l+1} = \textbf{h}_{i}^{l} + \mathrm{mean}_{j\in \mathcal{N}(i)}\left(\left\{(W_e\cdot \textbf{e}_{i,j} + b_e) \cdot \textbf{h}_j^{l} \right\}\right),
\end{equation}
where $\mathrm{mean}(\cdot)$ refers to the mean aggregation function in GCN. %\sz{What specific aggregation function do we use?} 
$h_i^l$ refers to the embedding of $i$-th node at layer $l$. $W_e$ and $b_e$ are the linear transformation parameters for the input edge features $\textbf{2}_{i,j}$. $\mathcal{N}(i)$ refers to the neighboring node set to the node $i$.

\textbf{\emph{Edge-based attention:}}. In GCNs, it is well known that attention allows for the efficient assignments of different weights to the connected edges of a node, which endows the interpretability on the importance of those edges to that node~\cite{velivckovic2017graph,wang2019kgat,wang2019heterogeneous}.
In our case, since utterances characterize customer-skill interactions, and attention is used to determine the weights of such interactions, we can also introduce the utterance factor into the attention module to control the generation of attention weights. This way, the attention weights would reflect the importance of such utterance as compared to all other utterances connected to the same node. Please refer to Eq.~\ref{GATConv1}-\ref{GATConv3} below for details:

\begin{equation}
\label{GATConv1}
\textbf{h}_i^{l+1} = \sum_{j\in \mathcal{N}(i)} \alpha_{i,j} W^{l} \textbf{h}_j^{l},
\end{equation}

\begin{equation}
\label{GATConv2}
 \alpha_{i,j}^{l} = \mathrm{softmax} (k_{i,j}^{l}),
\end{equation}

\begin{equation}
\label{GATConv3}
 k_{i,j}^{l} = \mathrm{LeakyReLU}\left(\vec{a}^T [W_a[ \textbf{h}_{i}^l\|\textbf{e}_{i,j}] \| W_a[\textbf{h}_{j}^l\|\textbf{e}_{i,j}]]\right),
\end{equation}
where $W_a$ and $W^l$ are the linear encoding matrix for attention module and for message passing at layer $l$, respectively. $\alpha_{i,j}$ and $\vec{a}$ refer to the attention weights and linear encoding vector for attention module, respectively. $[\cdot \| \cdot]$ refers to the concatenation operator.

\subsection{Personalizer}
The typical output of GCN model is node embeddings.
However, these node embeddings are too generic to be used for context-sensitive applications as ours.
For example, the link prediction objective, shown in Section~\ref{problem_define}, predicts the edge between a customer and a skill using simple inner product without having any context considerations. To resolve this problem, we design a new mechanism to provide the context-tailored customer embedding based on the learned customer embedding and utterance.
We denote this mechanism as a \textit{Personalizer}.
Formally speaking,
\begin{equation}
\label{eqn:personalizer}
\textbf{h}_s^p = f_p([\textbf{h}_s^l\|utt])
\end{equation}
where $\textbf{h}_s^p$ is context-considered customer embedding, $f_p$ is a \textit{personalizer} function, and $utt$ is the utterance text that we would like to consider.
% As previously mentioned in section~\ref{intro}, it is hard to directly use the existing edge convolution operators to make node embeddings of customers distinguishable from different utterances.
% To overcome this issue, we propose a personalizer designed to personalize the node embedding of a customer by different utterances he/she initiates.
In this paper, we modeled $f_p$ to be a 2-layer neural network.

This personalized embedding $\textbf{h}_s^p$ replaced the conventional context-free customer embedding $\textbf{h}_u^L$ in link prediction objective (Section~\ref{problem_define}), as well as replacing the customer embedding in the down-stream task.
Note that, this mechanism is trained during the representation learning time and not the downstream task training time.

Overall, Figure~\ref{fig:model_diagram}illustrates the pipeline for the PDRFE model.

\begin{figure*}%[ht]
\includegraphics[width=1.0\linewidth]{figures/diagram1.png}
\caption{Diagram of PDRFE Pipeline}
\label{fig:model_diagram}
\end{figure*}



% % (see Figure~\ref{personalizer_diagram}). %\sz{what is conditional neural network, add a reference or use some other popular terms}. 
% This way, different customers, given same utterance embedding will result in different personalized embedding. And same customer will generate different personalized embedding by having different utterances. %Mathematically, the personalized embedding can be obtained with the following objective (Eq.~\ref{personalizer_obj}):

% \sz{add a formula to compute the personalized embeddings} \hs{thought about this before, but feel that having an equation is not as clear as just putting this diagram.}

% \begin{figure}[ht]
% \includegraphics[width=1.0\linewidth]{figures/personalizer_diagram.png}
% \caption{Diagram for the Personalizer}
% \label{personalizer_diagram}
% \end{figure}



% [PENDING]
% \subsection{Contrastive Learning Constraint}
% \hs{pending for a discussion on whether to include this part for this submission or to put it in the future work.}

% Here we choose to use contrastive learning to make skills of similar functionalities to be closer in the embedding space since it is well-aligned with our problem.
% It is often considered in contrastive learning to maximize pairs of embedding with similarity. \sz{again, making a choice in method based on popularity is not scientific. Revise the reasons why we need contrastive learning.}
% In our case, it’s corresponding to 1p and 3p skills that have similar functions \sz{why? Please be more specific}.
% In contrastive learning, we need to have positive and negative pairs for 1p and 3p skills.
% \jo{Here, we try to measure the similarity between 1p and 3p skills and used it for deciding positive and negative pairs.}
% \sout{Since there is no metadata for the similarity measure between 1p and 3p skills, o}One natural way is to consider their connected utterances. Formally speaking, a pair of skills is similar when they maintain a similar distribution of their connected utterances.
% \sout{Since we obtain the utterance embeddings through the HypRank model, we are able to obtain a high-dimensional distribution of utterances for every skill that represents the skill's identity.}
% \sout{To measure the closeness between skills, we measure the distance between the utterance distribution via maximum mean discrepancy (MMD) \sz{why use MMD?}, a kernel based used to measure the distance between high-dimensional distributions.}
% \jo{We used Maximum Mean Discrepancy (MMD), a kernel based method for measuring distance between high-dimensional distribution [cite].}
% \sout{To separate positive and negative pairs according to the MMDs, we use the following sign function:}
% \jo{The final positive and negative pair is decided by a threshold $\rho$ as follow.}
% \begin{equation}
% \label{sign_function}
% f(s_1, s_2) = \text{sign}(\text{MMD}(\text{Utt}(s_1), \text{Utt}(s_2)) - \rho),
% \end{equation}
% where $s_1$ and $s_2$ are two skills. $\text{MMD}(\cdot, \cdot)$ refers to the MMD \sout{distance calculator} taking the set of utterances, $\text{Utt}(\cdot)$, for both skill inputs. $\rho$ is the threshold \sout{function} that is chosen according to the overall histogram of MMDs of all skill pairs. \sout{And this is actually a hyperparameter that can be tuned during the modeling.} Here $f(s_1, s_2)=1$ indicates the two input skills are dissimilar--negative pair--, otherwise, they are similar--positive pair--.

% Once being able to identify the positive and negative pairs of skills, we can apply the contrastive learning constraint according to the following equation:
% \begin{equation}
% \label{cl_function}
% \sum_{s \in S_{1p}; \tilde{s}, \hat{s} \in S_{3p}} -\log \frac{\exp(\text{sim}(h_s^L, h_{\tilde{s}}^L)/\tau)}{\exp(\text{sim}(h_s^L, h_{\hat{s}}^L)/\tau) + \exp(\text{sim}(h_s^L, h_{\tilde{s}}^L)/\tau)},
% \end{equation}
% where $\tilde{s}$ and $\hat{s}$ refer to similar and dissimilar skills to the skill $s$. $S_{1p}$ and $S_{3p}$ are skill node sets for 1p and 3p skills, respectively. $\text{sim}(\cdot, \cdot)$ is a cosine similarity function and $\tau$ is a hyperparameter.




==> problem.tex <==
Here we formally define our problem in the context of graph representation learning: 

Given a bipartite customer-skill interaction graph $G=(V,E)$ where $V$ is the set of nodes and $E$ is the set of edges and $V=\{U,S\}$ where $U$ refers to the set of customer nodes and $S$ refers to the set of skill nodes and $e_{u,s}$ denotes that a service request from user $u$ is fulfilled by skill $s$ ($e_{u,s} \in E$) (Note that, here we simplify the notation, but there can be multiple interactions between a customer $u$ and a skill $s$). For simplicity, we use $\textbf{e}_{u,s}$ to represent the feature vector to the edge $e_{u,s}$. The objective is to design a model $f$ that maps the initial input embeddings $(\textbf{h}_u^0, \textbf{e}_{u,s}, \textbf{h}_s^0)$ of a graph to a set of final embedding vectors for both the user and skill nodes, denoted as $(\textbf{h}_u^L, \textbf{h}_s^L) = f(\textbf{h}_u^0, \textbf{e}_{u,s}, \textbf{h}_s^0)$, such that when incorporating these embeddings to the downstream task, the corresponding objective function is optimized. Here the superscript $L$ for both $\textbf{h}_u$ and $\textbf{h}_s$ indicates the output embeddings of both customers and skills from the GCN model $f$.  We choose the objective for representation learning as link prediction.
In short, we have: 
\begin{description}
  \item[$\bullet$ Input:] $G$
  \item[$\bullet$ Output:] $\textbf{h}_u^L , \textbf{h}_s^L$ for all $u,s \in V$
  \item[$\bullet$ Link prediction:] $\sum_{u\in U}\sum_{s \in \mathcal{N}^+(u), \hat{s} \in \mathcal{N}^-(u)} \max( M - <\textbf{h}_u^L, \textbf{h}_s^L> + <\textbf{h}_u^L, \textbf{h}_{\hat{s}}^L>, 0)\label{obj:link_prediction}$
  \item[$\bullet$ Downstream task (defect prediction):] $\min_{\sigma} \frac{1}{|E|}\sum_{u \in U, s\ in S} CE(\sigma(\textbf{h}_u^L, \textbf{h}_s^L),y)$,
\end{description}
where $\sigma(\cdot,\cdot)$ is the defect classifier, and $<\cdot, \cdot>$ is the inner product. $\mathcal{N}^+(u)$ is positive neighbors - the set of skill node that are connected to the customer $u$ node, and $\mathcal{N}^-(u)$ is negative neighbors - the set of randomly sampled noise skill nodes that are not connected to the customer node $u$ in the graph $G$. $M$ is a hyperparameter for the link prediction objective,  $y$ is defect label, and $CE(\cdot, \cdot)$ is the cross-entropy loss function.

==> results.tex <==

In this section, we describe how we setup our experiment and the dataset for training/evaluation for both representation learning and downstream evaluation (Section~\ref{dataset}), defined the baseline models to compare our work with (Section~\ref{baseline}),  performed hyper-parameter tuning (Section~\ref{hyperparameter_setup}). We then present the results of our best performing model, and provide ablation study on the modules proposed in the previous section to demonstrate the effects of each of the modules to the downstream task.

%TT: Simplified and re-wrote above. No need to refer to each section, it is obvious. 

%In this section, we firstly describe the experiment setup that consists of three pieces: Section~\ref{baseline}: Baseline models to compare with; Section~\ref{dataset}: Dataset setup for training/evaluation for both representation learning and downstream evaluation; Section~\ref{hyperparameter_setup}: Hyperparameter setup. We then present the results of our best performing model (Section~\ref{model_comparisons}), and provide ablation study (Section~\ref{ablation_study}) on the modules proposed in the previous section to demonstrate the effects of each of the modules to the downstream task.

\subsection{Dataset Setup} \label{dataset}
In this section, we provide the details of the dataset preparation for both representation learning (a graph dataset) and downstream evaluation (a regular input-output dataset). Both datasets are generated from the raw customer-skill interaction logs. For privacy, we only provide a fake example for illustration purposes (see Table~\ref{fake_data_tab}). Additionally, we include metadata come with the interaction logs in Table~\ref{meta_data_tab}. These metadata will be used either in generating the initial node embeddings or for edge feature assignments. Note that the ``Defect" in Table~\ref{meta_data_tab} is an 0-1 binary label used for $y$, which is predicted by CPDR team, in the downstream evaluation.

\begin{table*}[ht]
  \caption{Fake Examples for Customer-Skill Interaction Log}
  \label{fake_data_tab}
  \centering
 \resizebox{\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
Customer ID (CID) & Skill ID (SID) & Utterance (interaction1)  & Utterance (interaction2) & … \\ \midrule
10xxxxx           & Help           & What happened to my music & Can you help me          & … \\
21xxxxxx          & Help           & What can I do today       & Can you do a tutorial    & … \\
21xxxxxx          & Communication  & No                        & Connect to my phone      & … \\
89xxxxx           & Help           & Can you do a tutorial     & I have feedback          & … \\
10xxxxx           & Communication  & Drop in all devices       & Connect to my phone      & … \\
…                 & …              & …                         & …                        & … \\
    \bottomrule
  \end{tabular}}
\end{table*}


\begin{table*}[ht] 
\hspace*{-4cm}
  \caption{Metadata in the Customer-Skill Interaction Logs}
  \label{meta_data_tab}
  \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lllll}
\toprule
Name of Metadata      & Description                                                                            & Cardinality & Example                                                                               & Usage                                                                                                  \\ \midrule
Skill\_category       & Category of skills                                                                     & 22          & \begin{tabular}[c]{@{}l@{}}Social / \\ Education \& reference\end{tabular}            & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}For initializing\\ skill node\\ embeddings\end{tabular}}    \\
Skill\_type           & Skill type                                                                             & 7           & CUSTOM                                                                                &                                                                                                        \\
Skill\_subcategory    & Subcategory of skills                                                                  & 69          & \begin{tabular}[c]{@{}l@{}}Education \& Reference / \\ Social Networking\end{tabular} &                                                                                                        \\
Reporting\_category   & General category                                                                       & 28          & Education / Social                                                                    &                                                                                                        \\ \hline
wbr\_cor              & Weekly business review country                                                         & 19          & US / ROW                                                                              & \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}For initializing\\ customer node\\ embeddings\end{tabular}} \\
is\_prime             & Prime membership?                                                                      & 2           & Y / N                                                                                 &                                                                                                        \\
is\_amu               & Amazon music subscriber?                                                               & 2           & Y / N                                                                                 &                                                                                                        \\
is\_smart\_home\_cust & Smart home customer ?                                                                  & 2           & Y / N                                                                                 &                                                                                                        \\ \hline
Utterance             & Utterances (users’ requests)                                                           & N/A         & Play tiktok                                                                           & \multirow{2}{*}{Edge features}                                                                         \\
Defect                & \begin{tabular}[c]{@{}l@{}}Whether a request is\\  fulfilled successfully\end{tabular} & 2           & 1 / 0                                                                                 &                                                  \\ \bottomrule                                                     
\end{tabular}}
\end{table*}

\subsection{Baselines}
\label{baseline}
In order to verify the performance of our proposed model, we compare it with 4 baseline models. Here we list all these models in Table~\ref{baseline_tab} with reasons of selection.

% \begin{table}
%   \caption{Baseline Models}
%   \label{baseline_tab}
%   \centering
%   \begin{tabular}{l|ll}
%     \toprule
%     Model Name     & Description     & Reason of the Choice \\
%     \midrule
%     PinSage & PinSage is a large scale GCN model designed by Pinterest for recommending pins (images) to people. Considered only one node type  & $\sim$100     \\
%     Revised PinSage     & Output terminal & $\sim$10      \\
%     Rational Graph Convolutional Network (RGCN)     & Cell body       & up to $10^6$  \\
%     Raw One-hot Encoding     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table*}[ht]
  \caption{Baseline Models}
  \label{baseline_tab}
 \resizebox{\textwidth}{!}{
\begin{tabular}{l|ll}
\toprule
Model Name                                                                                & Description                                                                                                                                                                    & Reason of the Choice                                                                                                      \\ \hline
PinSage~\cite{ying2018graph}                                                                                   & \begin{tabular}[c]{@{}l@{}}PinSage is a large scale GCN model designed\\  by Pinterest for recommending pins (images) \\ to people. Considered only one node type\end{tabular} & \begin{tabular}[c]{@{}l@{}}Representation learning model\\  that has been applied to \\ real-world scenarios\end{tabular} \\ \hline
Revised PinSage                                                                           & \begin{tabular}[c]{@{}l@{}}Extend PinSage to 2 types of nodes\\  (both customer and skill)\end{tabular}                                                                        & \begin{tabular}[c]{@{}l@{}}Improve the original PinSage\\  for comparison in our case\end{tabular}                        \\ \hline
\begin{tabular}[c]{@{}l@{}}Rational Graph \\ Convolutional Network \\ (RGCN)~\cite{schlichtkrull2018modeling} \end{tabular} & Simple GCN designed for link prediction                                                                                                                                        & Baseline for link prediction                                                                                              \\ \hline
Raw One-hot Encoding                                                                      & \begin{tabular}[c]{@{}l@{}}No Training, just use one-hot encoder on\\  the user/skill metadata and use these for\\  the downstream task\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}Baseline for non-graph-based \\ approach\end{tabular}                                                                                      \\ 
\bottomrule
\end{tabular}}
\end{table*}

\subsubsection{Representation Learning}
\label{RL}

%\sz{changed three steps to two steps}
To prepare the graph for representation learning, firstly we subsample our dataset following these three steps to obtain a subsampled interaction log: 1) Randomly subsample 10\% customers by their customer ID (CID). 2) Collect all the interactions corresponding to the subsampled CIDs in 14-day logs. Then we turn this log into a graph by treating each interaction log as an edge in the graph connecting the corresponding customer and skill nodes. Overall, the processed graph contains 107,480,710 number of customer-skill interactions (e.g. edges) for 12,031,327 customers (e.g. customer node) and 8,110 skills (e.g. skill node). 

To train and evaluate the representation model, we randomly split this graph to two subgraphs based on uniform edge sampling. We sample 80\% edges for training graph and the other 20\% for testing graph.


\subsubsection{Downstream Evaluation}
Once the representation model is trained, we would generate embeddings for all the nodes, including personalized embeddings. We then convert the graph back into the customer-skill interaction log table with the only change udated to the personalized embeddings for given customer, skill and the corresponding utterance (e.g. $\textbf{e}_{i,j}$). We randomly split the dataset into train/validation/test sets in the standard way with split ratios being 6:2:2. The data are then evaluated with the proposed downstream objective (see Section~\ref{problem_define}).
% \sz{what's the ratio in label distribution?} \hs{this part I didn't record the number, it needs some check in the dataset and I don't have the access now}


\subsection{Hyperparameter Setup}
\label{hyperparameter_setup}
The following hyperparameter setup (shown in Table~\ref{hyperparameter_tab}) is applied for the representation learning and the downstream evaluation. %We choose these hyperparameters according to a sensitivity check on the RGCN model (shown in Figure~\ref{sensitivity_check}). We found that the change of hyperparameters do not affect the learned representations in terms of the downstream evaluation. As a result, we choose to use the one set of hyperparameter that maximizes the modeling speed (with maximum possible batch size). 
For the downstream evaluation, we use two classifiers: 1) logistic regression module being the linear classifier 2) A nonlinear classifier which consists of a 2-layer neural network with ReLU being the activation function. The hidden dimension for this network is 32. We choose to use a small number for the hidden dimension to avoid overfitting of this nonlinear classifier. This forces the learned representation to be high quality.


\begin{table}[ht]
  \caption{Hyperparameter Steup}
  \label{hyperparameter_tab}
  \centering
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Hyperparameter}                             & \multicolumn{2}{c}{Model}                                                                                                                                                \\ \cline{2-3} 
                                                            & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Representation \\ Learning\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Defect\\ Prediction\end{tabular}} \\ \midrule
Batch Size                                               & \begin{tabular}[c]{@{}c@{}}512/1024/\\ 2048/4096 \\ ($\times$5 for negative sampling)    \end{tabular}                          & 256                                                                             \\
Learning Rate                                               & 10\textasciicircum{}\{-4\}                                                             & 10\textasciicircum{}\{-4\}                                                      \\
\begin{tabular}[c]{@{}l@{}}Hidden \\ Dimension\end{tabular} & 128                                                                                    & 32                                                                              \\
Total \# of Epochs                                          & $\leq$ 10                                                                              & \begin{tabular}[c]{@{}c@{}}When validation \\ loss is stable\end{tabular}      \\ \bottomrule
\end{tabular}
\end{table}


% \begin{figure}
% \centering
% \label{sensitivity_check}
% \includegraphics[width=.7\linewidth]{figures/sensitivity_check.pdf}
% \caption{Hyperparameter sensiticity check. Here we consider 4 different hyperparameters}
% \end{figure}

\begin{figure*}[ht]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/personalizer_v2.pdf}
         \caption{\textit{Personalizer}}
         \label{ablation:personalizer}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/attention_v2.pdf}
         \caption{Edge-based attention}
         \label{ablation:attention}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/edge_conv_v2.pdf}
         \caption{``NNConv''}
         
        
         \label{ablation:edge_conv}
     \end{subfigure}
     \hfill
    %  \begin{subfigure}[b]{0.75\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figures/legend.png}
    %      \caption{Legend}
         
        
    %      \label{ablation:legend}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.45\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figures/pending.pdf}
    %      \caption{Contrastive Learning}
    %      \label{ablation:CL}
    %  \end{subfigure}
        \caption{Ablation study on modules in PDRFE. The 3 bar-plots include the comparisons between the models with and without the modules discussed in the method section. Specifically, there are 3 modules included in this comparison: 1. The \textit{personalizer}; 2. The NNConv; 3. The edge-based attention. The reference models (in {\color{blue} blue}) are the models without the component, which is compared to the models with the component (in {\color{orange} orange}). The numbers reported in the figures are cross-entropies. The sub-captions indicate which module in PDRFE we compare with, and the tick labels indicate the name of the reference models with details in the legend Table~\ref{ben_model_tab}.}
        \label{ablation_study_fig}
\end{figure*}

% Please add the following required packages to your document preamble:
\begin{table}[]
\centering
\caption{Legend for Reference Models.}
 \label{ben_model_tab}
\begin{tabular}{@{}ll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Reference Model\\ Configuration\end{tabular}} & \multirow{2}{*}{Description}                             \\
                                                                                         &                                                          \\ \midrule
RGCN                                                                                     & The backbone RGCN model                                  \\
EC                                                                                       & The backbone RGCN + NNConv                               \\
EAtt                                                                                     & The backbone RGCN + edge-based attention                 \\
Per                                                                                      & The backbone RGCN + \textit{Personalizer} \\ \bottomrule
\end{tabular}
\end{table}

To conduct the experiments, we use an Amazon AWS cluster with V100 NVIDIA GPUs with the following libraries: PyTorch~\cite{NEURIPS2019_bdbca288}, DGL~\cite{wang2019deep} and ``"torch-two-sample"~\cite{torch_two_sample}.

\subsection{Model Comparisons}
\label{model_comparisons}

Here we present the comparison between the PDRFE model and the 4 baseline models. Results are evaluated according to the testing cross entropy for the downstream defect prediction task (refer to Table~\ref{overall_tab}). It is clear that the PDRFE models (with either the ``NNConv'' or the edge-based attention) obtain lower cross-entropy. The relative improvements in cross-entropy ranges between 15\% to 41\% for logistic regression model, and 19\% to 31\% for the 2-layer neural network model. In addition, it is obvious that the incorporation of the utterance embeddings into the model contribute to huge improvements for the downstream task. On one hand, the edge features improve the precision for node representations. On the other hand, the \textit{personalizer} resolves the two aforementioned ambiguities. Both components contribute to the out-performance of PDRFE over the baseline models.  

\begin{table*}[ht]
  \caption{Comparison between Our Best Models with the Baselines. Evaluation is based on the testing cross-entropy in the downstream evaluation. \textbf{Bold} numbers refer to the best results.}
  \label{overall_tab}
  \centering
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Models}      & \multicolumn{2}{c}{Cross-Entropy (lower the better)} \\ \cline{2-3} 
                                & \multicolumn{1}{l}{Logistic Regression} & \multicolumn{1}{l}{2-layer Neural Network}     \\ \midrule
PinSage (Baseline)              & 0.543                   & 0.441                      \\
Revised PinSage (Baseline)      & 0.519                   & 0.421                      \\
Raw One-Hot Encoding (Baseline) & 0.462                   & 0.424                      \\
RGCN (Baseline)                 & 0.372                   & 0.371                      \\
PDRFE (w/ ``NNConv'')            & \textbf{0.317}                   & \textbf{0.303}                   \\
PDRFE (w/ edge-based attention)  & \textbf{0.324}              & \textbf{0.302}  \\
\bottomrule
\end{tabular}
\end{table*}

\subsection{Ablation Study}
\label{ablation_study}
To study the individual effects of each module in PDRFE, we perform this ablation study on the 4 modules in PDRFE. Results are shown in Figure~\ref{ablation_study_fig}. It is shown that in all cases in this ablation study, the models that have the proposed components in PDRFE outperform the reference models where such components are removed. Specifically, the maximum performance boost for the 3 components are: 1) \textit{Personalizer}: 12\% 2) ``NNConv'': 19\% 3) Edge-based attention: 13\%. Each component can contribute to improvements in the defect prediction. However, when consider them jointly in PDRFE model, the performance is even better. This indicates the necessity of incorporating the edge features into the message passing as well as the \textit{personalizer} in the GCN model.
